A nonlinear bending theory for nematic LCE plates

In this paper, we study an elastic bilayer plate composed of a nematic liquid crystal elastomer in the top layer and a nonlinearly elastic material in the bottom layer. While the bottom layer is assumed to be stress-free in the flat reference configuration, the top layer features an eigenstrain that depends on the local liquid crystal orientation. As a consequence, the plate shows non-flat deformations in equilibrium with a geometry that non-trivially depends on the relative thickness and shape of the plate, material parameters, boundary conditions for the deformation, and anchorings of the liquid crystal orientation. We focus on thin plates in the bending regime and derive a two-dimensional bending model that combines a nonlinear bending energy for the deformation, with a surface Oseen-Frank energy for the director field that describes the local orientation of the liquid crystal elastomer. Both energies are nonlinearly coupled by means of a spontaneous curvature term that effectively describes the nematic-elastic coupling. We rigorously derive this model as a {\Gamma}-limit from three-dimensional, nonlinear elasticity. We also devise a new numerical algorithm to compute stationary points of the two-dimensional model. We conduct numerical experiments and present simulation results that illustrate the practical properties of the proposed scheme as well as the rich mechanical behavior of the system.

==> anchoring.tex <==
\subsection{Anchoring conditions}
\subsubsection{Proof of Lemmas~\ref{P:Gamma:Strong:Anchoring}--\ref{L:volstronganch}}
\begin{proof}[Proof of Lemma~\ref{P:Gamma:Strong:Anchoring}]
  Part (a) follows from Theorem~\ref{T2} (a), which in particular yields $n_h\wto n$ weakly in $H^1(\OmegaT;\R^3)$, and thus $\Phi_{BC}(x',n_h(x'))\wto \Phi_{BC}(x',n(x')$ thanks to the linearity of $\Phi_{BC}$ and the boundedness of the trace operator as an operator from $H^1(\OmegaT;\R^3)$ to $L^2(\Gamma_n\times(0,\frac12);\R^3)$. Part (b) follows from Lemma~\ref{L:stronger} with $n_h:=n$.
\end{proof}
%
\begin{proof}[Proof of Lemma~\ref{L:volweakanch}]
  We only present the proof for $\mathcal G_h$, since the argument for $\mathcal H_h$ is the same. Furthermore, we note that with regard to the compactness statement, there is nothing to prove, since $\mathcal G_h\geq\mathcal E_h$.

  \step{1 - Convergence of the weak anchoring terms.}

  We claim that for any sequence $(y_h,n_h)\in H^1(\Omega;\R^3)\times H^1(\OmegaT;\mathbb S^2)$ with $\det(\nabla_hy_h)>0$ a.e.~in $\Omega$, and
  \begin{equation}\label{eq:st:50c}
    (\nabla_hy_h,n_h)\to (R_y,n)\qquad\text{in }L^2\text{ for some }y\in H^2_{\rm iso}(S;\R^3),
  \end{equation}
  we have
  \begin{alignat}{2}\label{eq:st:50a}
    \lim\limits_{h\to 0}\int_{\OmegaT}    |\frac{\nabla_hy_h^\top n_h}{|\nabla_hy_h^\top n_h|}-\hat n_0|^2\rho =&\int_S|R^\top n-\hat n_0|^2\bar\rho,\\\label{eq:st:50b}
    \lim\limits_{h\to 0}\int_{\OmegaT}    |\frac{\nabla_hy_h^\top n_h}{|\nabla_hy_h^\top n_h|}\cdot\hat \nu|^2\rho =&\int_S|R^\top n\cdot\hat\nu|^2\bar\rho.
  \end{alignat}
  We only prove \eqref{eq:st:50a}, since the argument for \eqref{eq:st:50b} is similar. By passing to a subsequence, \eqref{eq:st:50c} holds pointwise a.e., thus, $|\frac{\nabla_hy_h^\top n_h}{|\nabla_hy_h^\top n_h|}-\hat n_0|^2\rho\to |R^\top n-\hat n_0|^2\rho$ pointwise a.e. By domindated convergence the latter holds strongly in $L^1(\OmegaT)$. Since on the right-hand side only $\rho$ is not independent of $x_3$, we conclude \eqref{eq:st:50a}.  

  \step{2 - Lower bound} Let $(y_h,n_h)\in H^1(\Omega;\R^3)\times H^1(\OmegaT;\mathbb S^2)$ be a sequence converging to $(y,n)\in H^2_{\iso}(S;\R^3)\times H^1(S;\mathbb S^2)$ strongly in $L^2$. We need to show
  %
  \begin{equation}\label{eq:st:50}
    \mathcal G_0(y,n)\leq\liminf\limits_{h\to 0}\mathcal G_h(y_h,n_h).
  \end{equation}
  %
  By passing to a subsequence, we may w.l.o.g.~assume that $\lim\limits_{h\to 0}\mathcal G_h(y_h,n_h)=\liminf\limits_{h\to 0}\mathcal G_h(y_h,n_h)<\infty$ and (in view of Theorem~\ref{T1} (a)) that
  \begin{equation*}
    (y_h,\nabla_h y_h,n_h)\to (y,R_y,n)\qquad\text{strongly in }L^2.
  \end{equation*}
  By \eqref{eq:st:50a} combined with Theorem~\ref{T1} (b), \eqref{eq:st:50} follows.

  \step{2 - Recovery sequence} Let $n_h:=n$ and let $y_h$ denote the recovery sequence of Lemma~\ref{L:stronger}. Then \eqref{eq:st:50c} holds, and we conclude with help of \eqref{eq:st:50b} that $\mathcal G_h(y_h,n_h)\to \mathcal G_0(y,n)$.
  
\end{proof}

\begin{proof}[Proof of Lemma~\ref{L:volstronganch}]
  We only present the proof for $\mathcal H_h$, since the argument for $\mathcal G_h$ is the same.

  \step{1 - Compactness} Since $\mathcal E_h\leq\mathcal H_h$, we may appeal to Theorem~\ref{T1} (a). In particular, we have $n_h\to n$ strongly in $L^2$ (for a subsequence), and it remains to show that the limit $n\in H^1(S;\mathbb S^2)$ satisisfies the strong anchoring condition $R_y^\top n=\hat n_0$ a.e.~in $S$. The latter can be seen as follows: By Step~1 in the proof of Lemma~\ref{L:volweakanch}, we have
  \begin{equation*}
    \frac12\int_S|R^\top n\cdot\hat\nu|^2\leq \lim_{h\to 0}\int_{\OmegaT}    |\frac{\nabla_hy_h^\top n_h}{|\nabla_hy_h^\top n_h|}\cdot\hat\nu|^2.
  \end{equation*}
  Since integral on the right-hand side is bounded from above by $h^\beta\mathcal H_h(y_h,n_h)$ and since $(y_h,n_h)$ is a sequence with equibounded energy, we conlude that $R^\top n\cdot\hat\nu=0$ a.e.

  \step{2 - Lower bound} W.l.o.g. we may assume that $\lim\limits_{h\to 0}\mathcal H_h(y_h,n_h)=\liminf\limits_{h\to 0}\mathcal H_h(y_h,n_h)<\infty$. Furthermore, in view Step~1 it suffices to consider the case when $(\nabla_hy_h,n_h)\to (R_y,n)$ in $L^2$ for some $y\in H^2_{\iso}(S;\R^3)$ and $n\in H^1(S;\mathbb S^2)$ satisfying the strong anchoring condition $R^\top_yn\cdot\hat\nu$. We conclude that $\mathcal H(y,n)=\mathcal E(y,n)$, and thus the lower bound follows from the elementary bound $\mathcal H_h(y_h,n_h)\geq \mathcal E_h(y_h,n_h)$ and the lower bound for $\mathcal E_h(y_h,n_h)$ of Theorem~\ref{T1} (b).

  \step{3 - Recover sequence} We start with approximating an admissible target configuration $(y,n)$ (which satisfies the strong anchoring condition in the definition of $\mathcal H$) by a configuration with a smooth isometry: For $k\in\N$ choose $y^k\in H^2_{\rm iso}(S;\R^3)\cap C^\infty(\bar S;\R^3)$ with
  \begin{equation}\label{eq:st:55}
    \|y^k-y\|_{H^2}\leq \frac1k,
  \end{equation}
  and consider $n^k:=R_{y^k} R_y^\top n$. Then $n^k\in H^1(S;\mathbb S^2)$ and $R_{y_k}^\top n^k\cdot\hat\nu=R_y^\top n\cdot\hat\nu=0$ satisfies the strong anchoring condition. Thus, $\mathcal H(y^k,n^k)=\mathcal E(y^k,n^k)$. Furtheremore, from \eqref{eq:st:55} we conclude that $n_k\to n$ strongly in $H^1$, and thus Lemma~\ref{L:cont} yields
  \begin{equation}\label{eq:st:55b}
    \lim\limits_{k\to\infty}|\mathcal H(n^k,y^k)-\mathcal H(y,n)|=0.
  \end{equation}
  Next, we construct the recovery sequence for $(y^k,n^k)$: As in the proof of Lemma~\ref{L:stronger}, we find with help of Proposition~\ref{P:approx} a sequence $(y^k_h)\subset H^1(\Omega;\R^3)$ such that with $n_h^k:=n^k$ we have
  \begin{align}\label{eq:st:56a}
    &\lim\limits_{h\to0}\mathcal E_h(y^k_h,n^k_h)=\mathcal E(y^k,n^k)\\\label{eq:st:56b}
    &(y^k_h,n^k_h)\to (y^k,n^k)\text{ in }L^2,\\\label{eq:st:56c}
    &\limsup\limits_{h\to 0}\|h^{-1/2}(\nabla_hy^k_h-R_{y^k})\|_{L^\infty}<\infty.
  \end{align}
  From \eqref{eq:st:56c} and since $0<\beta<1$, we infer that
  \begin{equation*}
    h^{-\beta}\int_{\OmegaT}    |\frac{(\nabla_hy_h^k)^\top n_h^k}{|(\nabla_hy_h^k)^\top n_h^k|}\cdot\hat\nu|^2\to 0.
  \end{equation*}
  Thus, combined with \eqref{eq:st:56a}, \eqref{eq:st:56b}, and \eqref{eq:st:55b}, we conlude that
  \begin{equation*}
    c_{k,h}:=|\mathcal H_h(y^k_h,n^k_h)-\mathcal H(y,n)|+\|y_h^k-y\|_{L^2}+\|n^k_h-n\|_{L^2}
  \end{equation*}
  satisfies $\limsup\limits_{k\to\infty}\limsup\limits_{h\to 0} c_{k,h}=0$. Hence, the sought for recovery sequence is obtained by extracting a suitable diagonal sequence.
\end{proof}

\subsubsection{Proofs of Lemmas~\ref{L:ext} \& \ref{L:weak:anchoring:with:boundary:slices}}

The proof of Lemma~\ref{L:ext} is a direct consequence of the following, more detailed statement:
% \begin{lemma}[canonical extension]
%   There exists $C>0$ and $\bar\sigma>0$ (only depending on $\Gamma_n$) such that the following properties hold:
%   \begin{enumerate}[(a)]
%   \item The map $\Psi:\Gamma_n\times(0,\sigma)\to\Gamma^{\bar\sigma}_n$, $(x',s)\mapsto x'-s\nu_S(x')$ is a homeomorphism and $\Gamma^{\bar\sigma}_n\subset S$.
%   \item (Canonical extension). For all $f\in H^1(\Gamma_n)$, the identity
%     \begin{equation*}
%       \bar f(\Psi(x',s))=f(x')\text{ for a.e. $(x',s)\in\Gamma_n\times(0,\bar\sigma)$},
%     \end{equation*}
%     defines a unique function $\bar f\in H^1(\Gamma_n^{\bar\sigma})$ with $\bar f=f$ on $\Gamma_n$ in the sense of trace, and for all $0<\sigma\leq\bar\sigma$,    
%     \begin{alignat*}{2}
%       \int_{\Gamma^\sigma_n}|\bar f|^2\,dx'\leq &C\sigma\int_\Gamma|f|^2\,d\mathcal H^1,\\
%       \int_{\Gamma^\sigma_n}|\nabla\bar f|^2\,dx'\leq &C\sigma\int_\Gamma|\nabla_{\rm tan}f|^2\,d\mathcal H^1.
%     \end{alignat*}
%   \item For all $f\in H^1(\Gamma^{\bar\sigma}_n)$ and $0<\sigma\leq\bar\sigma$, we have
%     \begin{equation*}
%       \Big|\int_{\Gamma^\sigma_n}|f|^2\,dx'-\sigma\int_{\Gamma_n}|f|^2\,d\mathcal H^1\,\Big|\leq C\,\sigma\int_{\Gamma^{\bar\sigma}_n}|f|^2+|\nabla f|^2\,dx'.
%     \end{equation*}
%   \end{enumerate}
% \end{lemma}
% \begin{proof}
%   In the following $C>0$ denotes a constant that may change from line to line, but that can be chosen only depending on $\Gamma_n$.  We only present the proof in the case where $\Gamma_n$ admits a global parametrization, i.e., in the case, when there exists an arc-length parametrized $C^2$-curve $\gamma:(a,b)\to\R^2$ that homoeomorphically maps $(a,b)$ onto $\Gamma_n$. The general case can be reduced to this situation by the usual localization argument with help of a partition of unity and a countable atlas.

%   \step{1 - Proof of (a) and (b)}

%   Note that we have $\nu_S(\gamma(t))=R^\perp\gamma'(t)$ for all $t\in(a,b)$, where $R^\perp\in\SO 2$ denotes a fixed rotation by $90^\circ$. We consider the map $\Phi:(a,b)\times(-\bar\sigma,\bar\sigma)\to\R^2$, $\Phi(t,s):=\gamma(t)+sR^\perp\gamma'(t)$. From $\gamma\in C^2$ we get $\Phi\in C^1((a,b)\times(-\bar\sigma,\bar\sigma))$ and
%   \begin{equation*}
%     J_\Phi(t,s)=(\gamma'(t)+s R^\perp\gamma''(t),R^\perp\gamma'(t)),\quad \det(J_\Phi(t,s))=(1+s\kappa(t)),\quad \kappa(t):=R^\perp\gamma''(t)\cdot\gamma'(t).
%   \end{equation*}
%   Since $|\gamma''|$ is bounded by assumption, for $C$ sufficiently large and all $\sigma\in(0,\frac1C)$ we conclude that $\Phi$ is a $C^1$-diffeomorphism,
%   \begin{equation}\label{eq:st:80}
%    \|J_\Phi\|_\infty, \|J^{-1}_\Phi\|_\infty,\|\kappa\|_\infty\leq C,
%   \end{equation}
%   and
%   \begin{equation*}
%     \Phi(U_\sigma)=\Gamma^\sigma_n\subset S,\qquad U_\sigma:=(a,b)\times(-\sigma,0).
%   \end{equation*}
%   Since $\Phi(t,-s)=\Psi(\gamma(t),s)$ and because $\gamma:(a,b)\to\Gamma_n$ is a homeomorphism, part (a) follows. We conclude that $\bar f$ is well-defined, measurable and characterized by the identity
%   \begin{equation*}
%     \bar f(\Phi(t,s)):=f(\Phi(t,0))\qquad\text{for all }(t,s)\in U_\sigma.
%   \end{equation*}
%   Since $\Phi$ is a $C^1$-diffeomorphism and $f\in H^1(\Gamma_n)$, we conclude that $\bar f\in H^1(\Gamma^\sigma_n)$ and $\bar f=f$ in the sense of trace. The transformation rule for integrals yields
%   \begin{alignat*}{2}
%     \int_{\Gamma^\sigma_n}|\bar f|^2\leq C&\int_{U_\sigma}|\bar f\circ\Phi|^2= C\sigma \int_{a}^b|(f\circ\gamma)|^2=C\sigma\int_{\Gamma_n}|f|^2\,d\mathcal H^1.
%   \end{alignat*}
%   Furthermore, from the identity $\nabla\bar f\circ\Phi=J_\Phi^{-\top}\nabla(\bar f\circ\Phi)=(f\circ \gamma)'J_\Phi^{-\top}e_1$, the transformation rule, \eqref{eq:st:80}, and the identity $\int_{(a,b)}|(f\circ\gamma)'(t)|^2\,dt=\int_{\Gamma_n}|\nabla_{\rm tan}f|^2\,d\mathcal H^1$, we conclude
%   \begin{alignat*}{2}
%     \int_{\Gamma^\sigma_n}|\nabla\bar f|^2=&\int_{U_\sigma}|\nabla \bar f\circ\Phi|^2\det J_\Phi \leq C\int_{U_\sigma}|(f\circ\gamma)'|^2= C\sigma\int_{\Gamma_n}|\nabla_{\rm tan}f|^2\,d\mathcal H^1.
%   \end{alignat*}

%   \step{2 - Proof of (c)}

%   By the transformation rules for integrals we have
%   \begin{alignat*}{2}
%     &\int_{\Gamma^\sigma_n}|f|^2\,dx'-\sigma\int_{\Gamma_n}|f|^2\,d\mathcal H^1=\int_{U_\sigma}|f\circ\Phi|^2\det J_\Phi-|(f\circ\Phi)(t,0)|^2\,dsdt    \\
%     =&\int_{U_\sigma}\big(|f\circ\Phi|^2-|(f\circ\Phi)(t,0)|^2\big)\det J_\Phi\,dsdt+\int_{U_\sigma}|(f\circ\Phi)(t,0)|^2(1-\det J_\Phi)\,dsdt\\
%     =:&I_1+I_2.
%   \end{alignat*}
%   Hence, we only need to prove the following estimates
%   \begin{equation}\label{eq:st:71}
%     |I_1|\leq C\sigma \|f\|^2_{H^1(\gamma^\sigma_n)}\qquad\text{and}\qquad|I_2|\leq C\sigma \|f\|^2_{H^1(\gamma^\sigma_n)}.    
%   \end{equation}
%   We start with the estimate for $I_1$, and note that
%   \begin{alignat*}{2}
%     |I_1|\leq& C\left(\int_{U_\sigma}|(f\circ\Phi)(t,s)-(f\circ\Phi)(t,0)|^2\big)\,dsdt\right)^\frac12\left(\int_{U_\sigma}|f\circ\Phi|^2+|(f\circ\Phi)(t,0)|^2\big)\,dsdt\right)^\frac12\\
%     \leq& C(\|f\|_{L^2(\Gamma_n^\sigma)}+\sigma\|f\|_{L^2(\Gamma_n)})\left(\int_{U_\sigma}|(f\circ\Phi)(t,s)-(f\circ\Phi)(t,0)|^2\big)\,dsdt\right)^\frac12\\
%     \leq& C\|f\|_{H^1(\Gamma_n^\sigma)}\left(\int_{U_\sigma}|(f\circ\Phi)(t,s)-(f\circ\Phi)(t,0)|^2\big)\,dsdt\right)^\frac12,
%   \end{alignat*}
%   where for the last estimate we appealed to the trace estimate. We estimate the remaining term:
%   \begin{alignat*}{2}
%     &\int_{U_\sigma}|(f\circ\Phi)(t,s)-(f\circ\Phi)(t,0)|^2\leq\,\int_{U_\sigma}\big|\int_0^s\frac{d}{ds'}(f\circ\Phi)(t,s')\,ds'|^2\,dsdt\\
%     \leq\,& \int_{U_\sigma}|s|\int_0^{\sigma}|\frac{d}{ds'}(f\circ\Phi)(t,s')|^2\,ds'\,dsdt\,=\,\frac{\sigma^2}{2}\int_{U_\sigma}|\frac{d}{ds}(f\circ\Phi)|^2\,dsdt.
%   \end{alignat*}
%   Since $\frac{d}{ds}(f\circ\Phi)=\partial_s\Phi\cdot (\nabla f\circ\Phi)$ and thus $|\frac{d}{ds}(f\circ\Phi)|\leq |\nabla f\circ\Phi|$, we conclude
%   \begin{equation*}
%     \int_{U_\sigma}|(f\circ\Phi)(t,s)-(f\circ\Phi)(t,0)|^2\leq\,C\sigma^2\int_{\Gamma_n^\sigma}|\nabla f|^2\,dx',
%   \end{equation*}
%   and thus the first estimate of \eqref{eq:st:71} follows. For the second one, we note that $1-\det J_\Phi=s\kappa(t)$, and thus
%   \begin{equation*}
%     |I_2|\leq C\int_{U_\sigma}|(f\circ\gamma)(t)|^2|s|\,dsdt=\frac{C}{2}\sigma^2\int_{\Gamma_n}|f|^2
%   \end{equation*}
  
% \end{proof}
% \begin{lemma}
%   There exists a constant $C>0$ such that for all $0<\sigma\leq\frac1C$ and all $f\in H^1(\Gamma^\sigma_n)$ we have
% \end{lemma}
% \begin{proof}
  
% \end{proof}


% Suppose that $g_\sigma=0$ on $\Gamma_n$ in the sense of trace. Then Poincar\'e's inequality yields
% \begin{equation*}
%   \int_{\Gamma_n^\sigma}|g|^2\leq C\sigma^2 \int_{\Gamma_n^\sigma}|\nabla g|^2\,dx'.
% \end{equation*}
% Indeed, consider

% \begin{alignat*}{2}
%   &\int_a^b\int_{-\sigma}^0|N\circ\Phi(t,s)-N\circ\Phi(t,0)|^2(1+s\kappa(t))\,ds\,dt\\
%   =&\int_a^b\int_{-\sigma}^0|\int_0^s\frac{d}{ds}(N\circ\Phi)(t,s')\,ds'|^2\,ds\,dt\\
%   \leq &\frac{\sigma^2}{2}\int_a^b\int_{-\sigma}^0|\frac{d}{ds}(N\circ\Phi)(t,s')|^2\,ds'dt\\
%   \leq &\frac{\sigma^2}{2}\int_a^b\int_{-\sigma}^0|\nabla N(\Phi(t,s))|^2\,ds'dt\\
% \end{alignat*}

\begin{lemma}[Estimates for the canonical extension]\label{L:trace}
  There exists $C>0$ and $\bar\sigma>0$ (only depending on $\Gamma_n$) such that the following properties hold
  \begin{enumerate}[(a)]
  \item The map $\Psi:\Gamma_n\times(0,\bar\sigma)\to\Gamma^{\bar\sigma}_n$, $(x',s)\mapsto x'-s\nu_S(x')$ is a homeomorphism and $\Gamma^{\bar\sigma}_n\subset S$.
  \item The extension operator ${\rm E}:L^2(\Gamma_n)\to L^2(\Gamma_n^{\bar\sigma})$ defined by $({\rm E}f)(\Psi(x',s))=f(x')$ for a.e. $(x',s)\in\Gamma_n\times(0,\bar\sigma)$ is bounded and, in particular, satisfies for all $0<\sigma\leq\bar\sigma$,
    \begin{equation*}
      \Big|\,\frac{1}{\sigma}\int_{\Gamma^\sigma_n}|{\rm E}f|^2\,dx'-\int_{\Gamma_n}|f|^2\,d\mathcal H^1\,\Big|\leq C\sigma\int_{\Gamma_n}|f|^2\,d\mathcal H^1.
    \end{equation*}
  \item For all $f\in H^1(\Gamma^\sigma_n)$ and $g\in L^2(\Gamma_n)$ we have
    \begin{alignat*}{2}
      &\Big|\frac1\sigma\int_{\Gamma^\sigma_n}|f-{\rm E}g|^2\,dx'-\int_{\Gamma_n}|Tf-g|^2\,d\mathcal H^1\Big|\\
      \leq\,&C\Big(\|\nabla f\|_{L^2(\Gamma_n^\sigma)}\|f-{\rm E}g\|_{L^2(\Gamma_n^\sigma)}+\sqrt\sigma\|\nabla f\|_{L^2(\Gamma_n^\sigma)}\|Tf-g\|_{L^2(\Gamma_n)}+\sigma\|Tf-g\|_{L^2(\Gamma_n)}^2\Big),
    \end{alignat*}
    where $T:H^1(\Gamma_n^\sigma)\to L^2(\Gamma_n)$ denotes the trace operator.
  \end{enumerate}
\end{lemma}
\begin{proof}
  We only present the proof in the case where $\Gamma_n$ admits a global parametrization, i.e., in the case, when there exists an arc-length parametrized $C^2$-curve $\gamma:(a,b)\to\R^2$ that homoeomorphically maps $(a,b)$ onto $\Gamma_n$. The general case can be reduced to this situation by the usual localization argument with help of a partition of unity and a countable atlas. In the following $C>0$ denotes a constant that may change from line to line, but that can be chosen only depending on $\Gamma_n$. 
  
  \step{1 - Proof of (a)}

  Note that we have $\nu_S(\gamma(t))=R^\perp\gamma'(t)$ for all $t\in(a,b)$, where $R^\perp\in\SO 2$ denotes a fixed rotation by $90^\circ$. Set $U:=(a,b)\times(0,1)$ and define for $\sigma>0$, the surjection
  \begin{equation*}
    \Phi_\sigma:(a,b)\times (0,1)\to\Gamma_n^\sigma,\qquad \Phi_\sigma(t,s):=\gamma(t)-\sigma sR^\perp\gamma'(t).
  \end{equation*}
  Since $\gamma\in C^2$, we have $\Phi_\sigma\in C^1(U)$ and the Jacobian satisfies
  \begin{equation*}
    J_{\Phi_\sigma}(t,s)=(\gamma'(t)-\sigma s R^\perp\gamma''(t),-\sigma R^\perp\gamma'(t)),\quad |\det(J_{\Phi_\sigma}(t,s))|=\sigma|1-s\sigma\kappa(t)|,\quad \kappa(t):=R^\perp\gamma''(t)\cdot\gamma'(t).
  \end{equation*}
  Since $|\gamma''|$ is bounded by assumption, for $\bar\sigma>0$ sufficiently small and all $\sigma\in(0,\bar\sigma)$ we conclude that $\Phi_\sigma$ is a $C^1$-diffeomorphism and satisfies
  \begin{equation}\label{eq:st:80}
   \|J_{\Phi_\sigma}\|_\infty, \|J^{-1}_{\Phi_\sigma}\|_\infty,\|\kappa\|_\infty\leq C\quad\text{and}\quad    \Phi_\sigma(U)=\Gamma^\sigma_n\subset S.
 \end{equation}
 Note that
 \begin{equation}\label{eq:st:82}
   \Phi_\sigma(t,s)=\Psi(\gamma(t),\sigma s)\qquad\text{for all }(t,s)\in U.
 \end{equation}
 Since $\gamma:(a,b)\to\Gamma_n$ is an homeomorphism, part (a) follows.

 \step{2 - Proof of (b)}

 From \eqref{eq:st:82} and the definition of the extension ${\rm E}f$ we conclude that $({\rm E}f)(\Phi_\sigma(t,s))=(f\circ\Phi)(t,0)=(f\circ\gamma)(t)$. Since $\Gamma_n^\sigma=\Phi_\sigma(U)$, the transformation rule for integrals yields
 \begin{alignat*}{2}
   &\frac{1}{\sigma}\int_{\Gamma^\sigma_n}|{\rm E}f|^2\,dx' = \frac{1}{\sigma}\int_{U}|({\rm E}f)\circ\Phi_\sigma|^2|\det J_{\Phi_\sigma}|\,dsdt\\
   =&\,\int_U|f\circ\gamma|^2|1-\sigma s\kappa(t)|\,dsdt=\int_{\Gamma_n}|f|^2\,d\mathcal H^1+\int_U|f\circ\gamma|^2(|1-\sigma s\kappa(t)|-1)\,dsdt.
 \end{alignat*}
 Since $\|\kappa\|_\infty\leq C$, we conclude that ${\rm E}$ is bounded and the estimate of (b) follows.

 \step{3 - Proof of (c)}

 By density, we may assume w.l.o.g. that $f$ and $g$ are $C^1$.  Note that
 \begin{alignat*}{2}
   &\frac1\sigma\int_{\Gamma^\sigma_n}|f-{\rm E}g|^2\,dx'=\int_U|(f-{\rm E}g)\circ\Phi_\sigma|^2|1- \sigma s\kappa(t)|\,dsdt,\\
   &\frac1\sigma\int_{\Gamma^\sigma_n}|{\rm E}(Tf-g)|^2\,dx'=\int_U|((Tf-g)\circ\Phi_\sigma)(t,0)|^2|1- \sigma s\kappa(t)|\,dsdt\\
   =&\int_{\Gamma_n}|Tf-g|^2\,d\mathcal H^1+\int_U|(Tf-g)\circ\gamma|^2\big(|1- \sigma s\kappa(t)|-1)\,dsdt.
 \end{alignat*}
 Thus,
 \begin{alignat*}{2}
   &\frac1\sigma\int_{\Gamma^\sigma_n}|f-{\rm E}g|^2\,dx'-\int_{\Gamma_n}|Tf-g|^2\,d\mathcal H^1\\
   =&\int_U\big(|(f-{\rm E}g)\circ\Phi_\sigma|^2-|((Tf-g)\circ\Phi_\sigma)(t,0)|^2\big)|1-\sigma s\kappa(t)|\,dsdt\\
   & -\int_U|(Tf-g)\circ\gamma|^2\big(|1- \sigma s\kappa(t)|-1)\,dsdt\\
   =&I_1+I_2.
 \end{alignat*}
 We first note that $|I_2|\leq C\sigma\|Tf-g\|^2_{L^2(\Gamma_n)}$. For $I_1$ we appeal to the general estimate $\|A^2-B^2\|_{L^1}\leq(\|A\|_{L^2}+\|B\|_{L^2})\|A-B\|_{L^2}$, the identity ${\rm E}g\circ\Phi_\sigma=g\circ\Phi_\sigma(\cdot,0)$, and $\|\cdot\|_{L^2(U)}\leq C\sigma^{-\frac12}\|\cdot\|_{L^2(\Gamma^\sigma_n)}$:
 \begin{alignat*}{2}
   |I_1|&\leq C\big(\sigma^{-\frac12}\|f-{\rm E}g\|_{L^2(\Gamma_n^\sigma)}+\|Tf-g\|_{L^2(\Gamma_n)}\big)\left(\int_U|(f\circ\Phi_\sigma)(t,s)-(Tf\circ\Phi_\sigma)(t,0)|^2\,dsdt\right)^\frac12.
 \end{alignat*}
 Moreover, since $(f\circ\Phi_\sigma)(t,s)-(Tf\circ\Phi_\sigma)(t,0)=\int_0^s\partial_s(f\circ\Phi)(t,s')\,ds'$ and $|\partial_s(f\circ\Phi_\sigma)|\leq C\sigma|\nabla f\circ\Phi_\sigma|$, we get
 \begin{alignat*}{2}
   &\int_U|(f\circ\Phi_\sigma)(t,s)-(Tf\circ\Phi_\sigma)(t,0)|^2\,dsdt\\
   \leq&\int_U\int_0^s|\partial_s(f\circ\Phi_\sigma(t,s'))|^2\,ds'\,dsdt\,\leq\,C\sigma^2\int_U|\nabla f\circ\Phi_\sigma|^2\,ds'dt\\
   \leq & C\sigma\int_{\Gamma^\sigma_n}|\nabla f|^2\,dx'.
 \end{alignat*}
\end{proof}

\begin{proof}[Proof of Lemma~\ref{L:weak:anchoring:with:boundary:slices}]
  We only present the argument for $\mathcal G^\sigma$, since $\mathcal H^\sigma$ can be treated similarly. Part (a) directly follows from Lemma~\ref{L:volweakanch}.

  \step{1 -- Proof of (b), lower bound} Let $\alpha=0$ and consider a sequence $(y_\sigma,n_\sigma)$   that converges to some $(y,n)$ in $L^2$. W.l.o.g.~we may assume that $\liminf\limits_{\sigma\to 0}\mathcal G^\sigma(y_\sigma,n_\sigma)=\limsup\limits_{\sigma\to 0}\mathcal G^\sigma(y_\sigma,n_\sigma)<\infty$.  Thus, Lemma~\ref{L:cont} implies that $(y_\sigma,n_\sigma),(y,n)\in \mathcal A_2$, $y_\sigma\wto y$ weakly in $H^2$, $n_\sigma\wto n$ weakly in $H^1$, and $\liminf_{\sigma\to 0}\mathcal E(y_\sigma,n_\sigma)\geq\mathcal E(y,n)$. It thus remains to prove
  \begin{equation}\label{eq:st:90}
    \liminf\limits_{\sigma\to 0}\frac1\sigma\int_{\Gamma^\sigma_n}|R_{y_\sigma}^\top n_\sigma-{\rm E}\hat n_{BC}|^2\geq \int_{\Gamma_n}|T(R_y^\top n)-n_{BC}|^2,
  \end{equation}
  where $T:H^1(S;\R^3)\to L^2(\Gamma_n;\R^3)$ denotes the trace operator.
  For convenience set $f_\sigma:=R_{y_\sigma}^\top n_{\sigma}$. We note that $(f_\sigma)$ is a bounded sequence in $H^1(S;\R^3)$. Thus, by the continuity of the trace operator, we deduce that 
  \begin{equation*}
    \|\nabla f_\sigma\|_{L^2(S)}+    \|T f_\sigma\|_{L^2(\Gamma_n)}\leq C;
  \end{equation*}
  where here and below $C$ denotes a positive constant that might change from line to line, but that can be chosen independently of $\sigma$. Combined with  Lemma~\ref{L:trace} we get
  \begin{equation}
    \label{eq:st:91}
    \Big|\frac1\sigma\int_{\Gamma^\sigma_n}|f_\sigma-{\rm E}\hat n_{BC}|^2\,dx'-\int_{\Gamma_n}|Tf_\sigma-\hat n_{BC}|^2\,d\mathcal H^1\Big|\,\leq\,C\sqrt{\sigma}\Big(\sigma^{-\frac12}\|f_\sigma-{\rm E}\hat n_{BC}\|_{L^2(\Gamma_n^\sigma)}+1\Big).
  \end{equation}
  Since $\sigma^{-\frac12}\|f_\sigma-{\rm E}\hat n_{BC}\|_{L^2(\Gamma_n^\sigma)}\leq\mathcal (\mathcal G^{\sigma}(y_\sigma,n_\sigma))^\frac12$, we infer that
  \begin{equation*}
    \liminf\limits_{\sigma\to 0}\sigma^{-1}\int_{\Gamma^\sigma_n}|R_{y_\sigma}^\top n_\sigma-{\rm E}\hat n_{BC}|^2=\liminf\limits_{\sigma\to0 }\int_{\Gamma_n}|Tf_\sigma-n_{BC}|^2.
  \end{equation*}
  Now, the  statements follows from the fact that $f_\sigma\wto R_y^\top n$ weakly in $H^1(S;\R^3)$, and thus $Tf_\sigma-\hat n_{BC}\wto Tf-\hat n_{BC}$ weakly in $L^2(\Gamma_n;\R^3)$, and the weak lower semicontinuity of $\|\cdot\|_{L^2(\Gamma_n)}$.

  \step{2 -- Proof of (c), lower bound} Let $0<\alpha<\frac12$ and consider a sequence $(y_\sigma,n_\sigma)$ that converges to some $(y,n)$ in $L^2$. As in Step~1 we may assume w.l.o.g.~that $\liminf_{\sigma\to 0}\mathcal G^\sigma(y_\sigma,n_\sigma)=\limsup_{\sigma\to 0}\mathcal G^\sigma(y_\sigma,n_\sigma)<\infty$,  $(y_\sigma,n_\sigma),(y,n)\in \mathcal A_2$, $y_\sigma\wto y$ weakly in $H^2$, $n_\sigma\wto n$ weakly in $H^1$, and $\liminf_{\sigma\to 0}\mathcal E(y_\sigma,n_\sigma)\geq\mathcal E(y,n)$. Thanks to \eqref{eq:st:90} and $\frac1\sigma\int_{\Gamma^\sigma_n}|R_{y_\sigma}^\top n_\sigma-{\rm E}\hat n_{BC}|^2\leq \sigma^\alpha\mathcal G^\sigma(y_\sigma,n_\sigma)$, we conclude that the strong anchoring condition $R_y^\top n=\hat n_{BC}$ on $\Gamma_n$ is satisfied, and thus $\mathcal G^\infty(y,n)=\mathcal E(y,n)\leq \liminf_{\sigma\to 0}\mathcal E(y_\sigma,n_\sigma)\leq \liminf_{\sigma\to 0}\mathcal G^\sigma(y_\sigma,n_\sigma)$.

  \step{3 -- Proof of (b), upper bound} It suffices to construct a recovery sequence for $(y,n)$ with $\mathcal G^0(y,n)<\infty$, which implies that $(y,n)\in\mathcal A_2$. We claim that the constant sequence is a recovery sequence, i.e., we need to show that $\frac1\sigma\int_{\Gamma_n^\sigma}|R^\top_yn-{\rm E}\hat n_{BC}|^2\,dx'\to\int_{\Gamma_n}|T(R^\top_yn)-\hat n_{BC}|^2\,d\mathcal H^1$. The latter follows from \eqref{eq:st:91} applied with $f_\sigma=R^\top_yn$.
  
  \step{4 -- Proof of (c), upper bound} Let $(y,n)$ with $\mathcal G^\infty(y,n)<\infty$. The latter implies that $(y,n)\in\mathcal A_2$ and $R^\top_yn=\hat n_{BC}$ on $\Gamma_n$. We claim that the constant sequence is a recovery sequence. Indeed, from \eqref{eq:st:91} applied with $f_\sigma=R^\top_yn$ and thanks to $Tf_\sigma={\rm E}\hat n_{BC}$, we learn that
  \begin{alignat*}{2}
    \sigma^{-(1+\alpha)}\int_{\Gamma_n^\sigma}|R^\top_yn-{\rm E}\hat n_{BC}|^2\,dx'&\leq \sigma^{-\alpha}\Big|\frac1\sigma\int_{\Gamma_n^\sigma}|R^\top_yn-{\rm E}\hat n_{BC}|^2\,dx'-\int_{\Gamma_n}|T(R^\top_yn)-\hat n_{BC}|^2\,d\mathcal H^1\Big|\\
    &\leq C\left(\sigma^{\frac12-\alpha}+\sigma^\frac\alpha2\Big(\sigma^{-(1+\alpha)}\int_{\Gamma_n^\sigma}|R^\top_yn-{\rm E}\hat n_{BC}|^2\,dx'\Big)^\frac12\right).
  \end{alignat*}
  We conclude that $\sigma^{-(1+\alpha)}\int_{\Gamma_n^\sigma}|R^\top_yn-{\rm E}\hat n_{BC}|^2\,dx'\to 0$. Combined with Lemma~\ref{L:cont} we conclude that
  \begin{equation*}
    \lim\limits_{\sigma\to 0}\mathcal G^\sigma(y,n)=\mathcal E(y,n)=\mathcal G^\infty(y,n).
  \end{equation*}
\end{proof}


